Fast, Anytime Motion Planning for Prehensile Manipulation in Clutter

Many methods have been developed for planning the motion of robotic arms for picking and placing, ranging from local optimization to global search techniques, which are effective for sparsely placed objects. Dense clutter, however, still adversely affects the success rate, computation times, and quality of solutions in many real-world setups. The current work integrates tools from existing methodologies and proposes a framework that achieves high success ratio in clutter with anytime performance. The idea is to first explore the lower dimensional end effector's task space efficiently by ignoring the arm, and build a discrete approximation of a navigation function, which guides the end effector towards the set of available grasps or object placements. This is performed online, without prior knowledge of the scene. Then, an informed sampling-based planner for the entire arm uses Jacobian-based steering to reach promising end effector poses given the task space guidance. While informed, the method is also comprehensive and allows the exploration of alternative paths over time if the task space guidance does not lead to a solution. This paper evaluates the proposed method against alternatives in picking or placing tasks among varying amounts of clutter for a variety of robotic manipulators with different end-effectors. The results suggest that the method reliably provides higher quality solution paths quicker, with a higher success rate relative to alternatives.

==> 05_properties.tex <==
% This section provides a sketch of the arguments that can be made about
% the asymptotic optimality of the algorithm.

% \begin{proposition}
% \label{prop:coverage}
% $ \mathtt{JIST} $ is guaranteed to eventually reach the optimal
% grasping state.  \\ \noindent\textit{Sketch:} Prior work
% \cite{berenson2010probabilistically} has argued that a pseudo-inverse
% projection operator can be used to guarantee a probabilistically
% complete mapping of $\cfull$ to the end effector pose space
% $\mathbb{E}$. Using $ \mathbb{J}^+steering $ and
% Eq. \ref{equ:jacsteering} ensures asymptotically complete coverage of
% $\mathbb{Q}_{goal}$, while the fallback edges allow the reachable
% subset of $\mathbb{Q}_{goal}$ to be connected to the search tree with
% alternative paths.


% % Use of a $ \mathbb{J}^+steering $ projection ensures an asymptotically complete coverage of the goal manifold. 
% % Once a goal state is projected to, it is saved so that a fallback maneuver can attempt a connection to it.
% \end{proposition}

% \begin{proposition}
% \label{prop:convergence}
% The cost of a path that observes the optimal solution path converges to the optimal cost.
% \\ \noindent\textit{Sketch:} A sequence of finite hyperballs of radius $ \delta $ can be
% constructed to tile the optimal solution path that has the lowest cost. A path that observes the optimal path is contained in
% these hyperballs and bears a Euclidean cost.

% $ \cdist $ forms a metric space \cite{zhang2007c} when computed over
% the end effector geometry. For a robotic arm with bounded reachability
% and a bounded $ \cfull$, there must exist a finite constant $ K_c $
% that bounds the ratio between the Euclidean cost and $ \cdist $ cost
% for the straight line between any pair of points in $ \cfull $.
% Assuming Lipschitz continuity of curves in $ \cfull $, the Euclidean
% cost of the observed path is bounded w.r.t. the cost of the observed
% path, and converges with reducing $ \delta $. Given the bounded
% continuity assumptions and for finite costs of the
% observing path and non-zero costs of the optimal path, this
% convergence holds for $ \cdist $.
% \end{proposition}



% \begin{proposition}
% \label{prop:ao}
% $ \mathtt{JIST} $ is asymptotically optimal.
% \\ \noindent\textit{Sketch:} A Markov chain is constructed that
% ``observes'' an optimal path and has an absorption state corresponding
% to the goal region. Then, if the probability of transitioning between
% Markov states is non-zero, the method surely reaches the absorbing
% state wtih infinite tries \cite{Snell2012} (Theorem 11.3).  Given a
% covering ball sequence for an optimal path $\pi^\ast$ with some
% $\delta$ clearance, \jist\ satisfies the following conditions:
% % A covering ball sequence for an optimal path
% % $\pi^\ast$ for some $\delta$ clearance of the optimal path is constructed. 


%  \noindent \emph{(1)} The subroutine $ \mathtt{SearchSelection} $ ensures that the probability of selecting a node is always non-zero.
 
%  \noindent \emph{(2)} There is a non-zero probability of moving from
%  one covering ball to the next once a node is selected. Prior work
%  (Theorem 17 in \cite{Li:2016}) proves this given assumptions about
%  smooth system dynamics. This is guaranteed to have positive
%  probability when the propagation is not biased during expansion. This
%  is achieved by Alg. \ref{algo:jist} through the random controls with
%  random duration as fallback edges. This ensures that the Euclidean
%  cost of the path converges.
 
%  \noindent \emph{(3)} The optimal goal state is guaranteed to be
%  discovered and optimally connected to the search tree by Proposition
%  \ref{prop:coverage}.
 
%  \noindent \emph{(4)} The cost of the observing path
%  converges to the optimal cost by Proposition
%  \ref{prop:convergence}.
  

% \end{proposition}

